Measurement of the effective $B^0_s\rightarrow K^+K^-$ lifetime

A measurement of the effective $B^0_s\rightarrow K^+K^-$ lifetime is presented using approximately $37 pb^{-1}$ of data collected by LHCb during 2010. This quantity can be used to put constraints on contributions from processes beyond the Standard Model in the $B^0_s$ meson system and is determined by two complementary approaches as $\tau_{B^0_s\to K^+K^-} = 1.440 \pm 0.096 (stat) \pm 0.008 (syst) \pm 0.003 (model) ps$.

==> LHCb_comma_separated_author.tex <==
LHCb Collaboration:
R. Aaij, C. Abellan Beteta, B. Adeva, M. Adinolfi, C. Adrover, A. Affolder, Z. Ajaltouni, J. Albrecht, F. Alessio, M. Alexander, G. Alkhazov, P. Alvarez Cartelle, A.A. Alves Jr, S. Amato, Y. Amhis, J. Anderson, R.B. Appleby, O. Aquines Gutierrez, F. Archilli, L. Arrabito, A. Artamonov , M. Artuso, E. Aslanides, G. Auriemma, S. Bachmann, J.J. Back, D.S. Bailey, V. Balagura, W. Baldini, R.J. Barlow, C. Barschel, S. Barsuk, W. Barter, A. Bates, C. Bauer, Th. Bauer, A. Bay, I. Bediaga, S. Belogurov, K. Belous, I. Belyaev, E. Ben-Haim, M. Benayoun, G. Bencivenni, S. Benson, J. Benton, R. Bernet, M.-O. Bettler, M. van Beuzekom, A. Bien, S. Bifani, A. Bizzeti, P.M. Bj\o rnstad, T. Blake, F. Blanc, C. Blanks, J. Blouw, S. Blusk, A. Bobrov, V. Bocci, A. Bondar, N. Bondar, W. Bonivento, S. Borghi, A. Borgia, T.J.V. Bowcock, C. Bozzi, T. Brambach, J. van den Brand, J. Bressieux, D. Brett, S. Brisbane, M. Britsch, T. Britton, N.H. Brook, H. Brown, A. B\"{u}chler-Germann, I. Burducea, A. Bursche, J. Buytaert, S. Cadeddu, J.M. Caicedo Carvajal, O. Callot, M. Calvi, M. Calvo Gomez, A. Camboni, P. Campana, A. Carbone, G. Carboni, R. Cardinale, A. Cardini, L. Carson, K. Carvalho Akiba, G. Casse, M. Cattaneo, M. Charles, Ph. Charpentier, N. Chiapolini, K. Ciba, X. Cid Vidal, G. Ciezarek, P.E.L. Clarke, M. Clemencic, H.V. Cliff, J. Closier, C. Coca, V. Coco, J. Cogan, P. Collins, A. Comerma-Montells, F. Constantin, G. Conti, A. Contu, A. Cook, M. Coombes, G. Corti, G.A. Cowan, R. Currie, B. D'Almagne, C. D'Ambrosio, P. David, I. De Bonis, S. De Capua, M. De Cian, F. De Lorenzi, J.M. De Miranda, L. De Paula, P. De Simone, D. Decamp, M. Deckenhoff, H. Degaudenzi, M. Deissenroth, L. Del Buono, C. Deplano, D. Derkach, O. Deschamps, F. Dettori, J. Dickens, H. Dijkstra, P. Diniz Batista, F. Domingo Bonal, S. Donleavy, F. Dordei, A. Dosil Su\'{a}rez, D. Dossett, A. Dovbnya, F. Dupertuis, R. Dzhelyadin, A. Dziurda, S. Easo, U. Egede, V. Egorychev, S. Eidelman, D. van Eijk, F. Eisele, S. Eisenhardt, R. Ekelhof, L. Eklund, Ch. Elsasser, D.G. d'Enterria, D. Esperante Pereira, L. Est\`{e}ve, A. Falabella, E. Fanchini, C. F\"{a}rber, G. Fardell, C. Farinelli, S. Farry, V. Fave, V. Fernandez Albor, M. Ferro-Luzzi, S. Filippov, C. Fitzpatrick, M. Fontana, F. Fontanelli, R. Forty, M. Frank, C. Frei, M. Frosini, S. Furcas, A. Gallas Torreira, D. Galli, M. Gandelman, P. Gandini, Y. Gao, J-C. Garnier, J. Garofoli, J. Garra Tico, L. Garrido, D. Gascon, C. Gaspar, N. Gauvin, M. Gersabeck, T. Gershon, Ph. Ghez, V. Gibson, V.V. Gligorov, C. G\"{o}bel, D. Golubkov, A. Golutvin, A. Gomes, H. Gordon, M. Grabalosa G\'{a}ndara, R. Graciani Diaz, L.A. Granado Cardoso, E. Graug\'{e}s, G. Graziani, A. Grecu, E. Greening, S. Gregson, B. Gui, E. Gushchin, Yu. Guz, T. Gys, G. Haefeli, C. Haen, S.C. Haines, T. Hampson, S. Hansmann-Menzemer, R. Harji, N. Harnew, J. Harrison, P.F. Harrison, J. He, V. Heijne, K. Hennessy, P. Henrard, J.A. Hernando Morata, E. van Herwijnen, E. Hicks, K. Holubyev, P. Hopchev, W. Hulsbergen, P. Hunt, T. Huse, R.S. Huston, D. Hutchcroft, D. Hynds, V. Iakovenko, P. Ilten, J. Imong, R. Jacobsson, A. Jaeger, M. Jahjah Hussein, E. Jans, F. Jansen, P. Jaton, B. Jean-Marie, F. Jing, M. John, D. Johnson, C.R. Jones, B. Jost, M. Kaballo, S. Kandybei, M. Karacson, T.M. Karbach, J. Keaveney, U. Kerzel, T. Ketel, A. Keune, B. Khanji, Y.M. Kim, M. Knecht, S. Koblitz, P. Koppenburg, A. Kozlinskiy, L. Kravchuk, K. Kreplin, M. Kreps, G. Krocker, P. Krokovny, F. Kruse, K. Kruzelecki, M. Kucharczyk, R. Kumar, T. Kvaratskheliya, V.N. La Thi, D. Lacarrere, G. Lafferty, A. Lai, D. Lambert, R.W. Lambert, E. Lanciotti, G. Lanfranchi, C. Langenbruch, T. Latham, R. Le Gac, J. van Leerdam, J.-P. Lees, R. Lef\`{e}vre, A. Leflat, J. Lefran\c{c}ois, O. Leroy, T. Lesiak, L. Li, L. Li Gioi, M. Lieng, M. Liles, R. Lindner, C. Linn, B. Liu, G. Liu, J.H. Lopes, E. Lopez Asamar, N. Lopez-March, J. Luisier, F. Machefert, I.V. Machikhiliyan, F. Maciuc, O. Maev, J. Magnin, S. Malde, R.M.D. Mamunur, G. Manca, G. Mancinelli, N. Mangiafave, U. Marconi, R. M\"{a}rki, J. Marks, G. Martellotti, A. Martens, L. Martin, A. Mart\'{i}n S\'{a}nchez, D. Martinez Santos, A. Massafferri, Z. Mathe, C. Matteuzzi, M. Matveev, E. Maurice, B. Maynard, A. Mazurov, G. McGregor, R. McNulty, C. Mclean, M. Meissner, M. Merk, J. Merkel, R. Messi, S. Miglioranzi, D.A. Milanes, M.-N. Minard, S. Monteil, D. Moran, P. Morawski, R. Mountain, I. Mous, F. Muheim, K. M\"{u}ller, R. Muresan, B. Muryn, M. Musy, J. Mylroie-Smith, P. Naik, T. Nakada, R. Nandakumar, J. Nardulli, I. Nasteva, M. Nedos, M. Needham, N. Neufeld, C. Nguyen-Mau, M. Nicol, S. Nies, V. Niess, N. Nikitin, A. Nomerotski, A. Novoselov, A. Oblakowska-Mucha, V. Obraztsov, S. Oggero, S. Ogilvy, O. Okhrimenko, R. Oldeman, M. Orlandea, J.M. Otalora Goicochea, P. Owen, K. Pal, J. Palacios, A. Palano, M. Palutan, J. Panman, A. Papanestis, M. Pappagallo, C. Parkes, C.J. Parkinson, G. Passaleva, G.D. Patel, M. Patel, S.K. Paterson, G.N. Patrick, C. Patrignani, C. Pavel-Nicorescu, A. Pazos Alvarez, A. Pellegrino, G. Penso, M. Pepe Altarelli, S. Perazzini, D.L. Perego, E. Perez Trigo, A. P\'{e}rez-Calero Yzquierdo, P. Perret, M. Perrin-Terrin, G. Pessina, A. Petrella, A. Petrolini, E. Picatoste Olloqui, B. Pie Valls, B. Pietrzyk, T. Pilar, D. Pinci, R. Plackett, S. Playfer, M. Plo Casasus, G. Polok, A. Poluektov, E. Polycarpo, D. Popov, B. Popovici, C. Potterat, A. Powell, T. du Pree, J. Prisciandaro, V. Pugatch, A. Puig Navarro, W. Qian, J.H. Rademacker, B. Rakotomiaramanana, M.S. Rangel, I. Raniuk, G. Raven, S. Redford, M.M. Reid, A.C. dos Reis, S. Ricciardi, K. Rinnert, D.A. Roa Romero, P. Robbe, E. Rodrigues, F. Rodrigues, P. Rodriguez Perez, G.J. Rogers, S. Roiser, V. Romanovsky, M. Rosello, J. Rouvinet, T. Ruf, H. Ruiz, G. Sabatino, J.J. Saborido Silva, N. Sagidova, P. Sail, B. Saitta, C. Salzmann, M. Sannino, R. Santacesaria, C. Santamarina Rios, R. Santinelli, E. Santovetti, M. Sapunov, A. Sarti, C. Satriano, A. Satta, M. Savrie, D. Savrina, P. Schaack, M. Schiller, S. Schleich, M. Schmelling, B. Schmidt, O. Schneider, A. Schopper, M.-H. Schune, R. Schwemmer, B. Sciascia, A. Sciubba, M. Seco, A. Semennikov, K. Senderowska, I. Sepp, N. Serra, J. Serrano, P. Seyfert, B. Shao, M. Shapkin, I. Shapoval, P. Shatalov, Y. Shcheglov, T. Shears, L. Shekhtman, O. Shevchenko, V. Shevchenko, A. Shires, R. Silva Coutinho, H.P. Skottowe, T. Skwarnicki, A.C. Smith, N.A. Smith, E. Smith, K. Sobczak, F.J.P. Soler, A. Solomin, F. Soomro, B. Souza De Paula, B. Spaan, A. Sparkes, P. Spradlin, F. Stagni, S. Stahl, O. Steinkamp, S. Stoica, S. Stone, B. Storaci, M. Straticiuc, U. Straumann, N. Styles, V.K. Subbiah, S. Swientek, M. Szczekowski, P. Szczypka, T. Szumlak, S. T'Jampens, E. Teodorescu, F. Teubert, C. Thomas, E. Thomas, J. van Tilburg, V. Tisserand, M. Tobin, S. Topp-Joergensen, N. Torr, E. Tournefier, M.T. Tran, A. Tsaregorodtsev, N. Tuning, M. Ubeda Garcia, A. Ukleja, P. Urquijo, U. Uwer, V. Vagnoni, G. Valenti, R. Vazquez Gomez, P. Vazquez Regueiro, S. Vecchi, J.J. Velthuis, M. Veltri, K. Vervink, B. Viaud, I. Videau, X. Vilasis-Cardona, J. Visniakov, A. Vollhardt, D. Voong, A. Vorobyev, H. Voss, K. Wacker, S. Wandernoth, J. Wang, D.R. Ward, A.D. Webber, D. Websdale, M. Whitehead, D. Wiedner, L. Wiggers, G. Wilkinson, M.P. Williams, M. Williams, F.F. Wilson, J. Wishahi, M. Witek, W. Witzeling, S.A. Wotton, K. Wyllie, Y. Xie, F. Xing, Z. Xing, Z. Yang, R. Young, O. Yushchenko, M. Zavertyaev, F. Zhang, L. Zhang, W.C. Zhang, Y. Zhang, A. Zhelezov, L. Zhong, E. Zverev, A. Zvyagin

